Low Resource Recognition and Linking of Biomedical Concepts from a Large Ontology

Tools to explore scientific literature are essential for scientists, especially in biomedicine, where about a million new papers are published every year. Many such tools provide users the ability to search for specific entities (e.g. proteins, diseases) by tracking their mentions in papers. PubMed, the most well known database of biomedical papers, relies on human curators to add these annotations. This can take several weeks for new papers, and not all papers get tagged. Machine learning models have been developed to facilitate the semantic indexing of scientific papers. However their performance on the more comprehensive ontologies of biomedical concepts does not reach the levels of typical entity recognition problems studied in NLP. In large part this is due to their low resources, where the ontologies are large, there is a lack of descriptive text defining most entities, and labeled data can only cover a small portion of the ontology. In this paper, we develop a new model that overcomes these challenges by (1) generalizing to entities unseen at training time, and (2) incorporating linking predictions into the mention segmentation decisions. Our approach achieves new state-of-the-art results for the UMLS ontology in both traditional recognition/linking (+8 F1 pts) as well as semantic indexing-based evaluation (+10 F1 pts).

==> 07_related_work.tex <==
%---------------------------------------------------------------------------------------------------
\section{Related Work}

In this section, we provide a summary of relevant related work, referring readers to Appendix~\S\ref{app:related-work} for a longer exposition. \citet{Kolitsas-etal:2018} also present a bottom-up end-to-end linking model. Our approach differs in two ways: (1) \citet{Kolitsas-etal:2018}'s work does not support low-resource settings where entities do not have description pages and sample hyperlinks, and (2) we incorporate linking decisions into the span selection component. The former makes \citet{Kolitsas-etal:2018} difficult to apply directly to MedMentions. We train each model component separately rather than jointly.

The Zeshel model \citep{Logeswaran-etal:2019} presents an approach for zero-shot entity linking that allows for linking mentions to entities unseen at training time. However, this work also relies on entity description resources, and they do not do entity recognition. Similar to Zeshel, our span linker and selector models use a trained vector to mark mention tokens.

Apart from the methods we compare to in this work, \citet{Murty-etal:2018:HierarchicalLoss}  and \citet{Zhu-etal:2020:LATTE} evaluate concept linking on MedMentions.
\citet{Zhu-etal:2020:LATTE}  use a latent type modeling layer, with type prediction as an auxiliary task. Bi-directional attention flow is used to compute the interaction between the contextualized mention and concept names, combining this with latent type similarity to get the final score.
However, both of these papers make the unrealistic assumption that the ground truth concept is in the set of candidates, making these methods not directly comparable to our work. 

The Large Scale Semantic Indexing Challenge tasks \citep{Nentidis-etal:2019:BioASQ} in the BioASQ\footnote{\url{http://bioasq.org}} workshops use a large dataset published by NCBI where documents are labeled with biomedical concepts from the MeSH ontology \citep{Lipscomb:2000:MeSH}, without identifying their mentions in the text. The ontology is much smaller than UMLS (fewer than 30k concepts), and its coverage in the training data is above 95\%, compared to less than 1\% coverage in MedMentions. Leading approaches treat this as a multi-label document classification problem \citep{Peng-etal:2016:DeepMeSH,Xun-etal:2019:MeSHProbeNet}.



==> AA_citations.tex <==
\nocite{Huang-etal:2015,Lample-etal:2016}
\nocite{FrancisLandau-etal:2016:BerkeleyCNN,Gupta-etal:2017:EMNLP}
\nocite{Li-etal:2015}
\nocite{Sachan-etal:2018}
\nocite{Kim-etal:2019:BERN}
\nocite{Nentidis-etal:2019:BioASQ}
\nocite{Lipscomb:2000:MeSH}
\nocite{Peng-etal:2016:DeepMeSH,Xun-etal:2019:MeSHProbeNet}
\nocite{Kolitsas-etal:2018}
\nocite{Murty-etal:2017}
\nocite{Logeswaran-etal:2019}
\nocite{Leaman-Zhiyong:2016}
\nocite{Mohan-Li:2019:AKBC}
\nocite{Murty-etal:2018:HierarchicalLoss}
\nocite{Zhu-etal:2020:LATTE}
\nocite{Murty-etal:2018:HierarchicalLoss}
\nocite{Nejadgholi-etal:2019}
\nocite{Lee-etal:2019:BioBERT}
\nocite{Loureiro-Jorge:2020:MedLinker}
\nocite{Mohan-Li:2019:AKBC}


==> figs/semantic_index.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/semantic_index_example.pdf}
    \caption{\textbf{Semantic Index for Biomedical Research Papers}: An example showing how relevant documents are retrieved based on the entities present in the text of the research papers. Entities labeled via entity recognition and linking systems.}
    \label{fig:example_semantic_index}
\end{figure}
% Edit this figure at: https://www.icloud.com/keynote/08UcTCJs9kTaTtxLJwNV8KYOg#2020-07-15-_Linking_Figure
